Linear Complexity Fermionic Simulation on Quantum Devices with Hardware Connectivity Constraints

Simulating fermionic systems on quantum hardware requires compiling fermionic Hamiltonians into executable quantum circuits. Existing approaches treat each compilation stage independently, applying heuristics with localized objectives that produce circuits with superquartic gate count and depth scaling and compilation times reaching several hours for large instances. We present Accordion, an end-to-end framework that co-designs the fermion-to-qubit mapping with circuit synthesis and hardware routing. Accordion fixes the Jordan Wigner mapping, which despite its higher Pauli weight produces Pauli operators with structural regularity that enables provably efficient circuit generation. For full-rank all-to-all electronic structure Hamiltonians, we prove O(N^4) gate count and circuit depth, matching the information-theoretic lower bound imposed by the Theta(N^4) second excitation terms. On linear, IBM heavy-hex, and square-grid architectures, Accordion reduces gate count by up to 79% and circuit depth by up to 77% relative to the best baseline.

==> Evaluation.tex <==
\section{Evaluation}
\label{sec:eval}
We evaluate \sysname{} by answering following questions.
\begin{enumerate}[label=Q\arabic*)]
    \item How effectively does \sysname{} reduce circuit depth and gate count?
    \item How well do these metrics scale with problem size?
    \item How efficient is our compiler runtime?
\end{enumerate} 
Q1 and Q2 are used to evaluate the quality of the compilation result, while Q3 reflects how fast users can obtain these results. 
We also provide a detailed breakdown analysis. 

\subsection{Experiment Setup}
\label{sec:experiment_setup}

\Para{Benchmarks}
We choose benchmarks of various sizes and applications from VQE 
and use the UCCSD ansatz~\cite{uccsd} for these benchmarks. 
The parameters of this ansatz are determined by several molecules retrieved from PubChem \cite{sunghwan2024pubchem} database. 
Specifically, we have constructed Hamiltonians with first and second excitation terms for 15 distinct molecules (e.g., LiH, $\text{BeH}_{2}$) utilizing the PySCF~\cite{PySCF} software package. 
More details for the selected molecules and resulting ansatz are presented in Table~\ref{tab:uccsd}.
Additionally, we generate all-to-all electronic Hamiltonians for $4\le n\le 40$ qubits to benchmark our approach's performance when every possible Pauli string is included to test the scalability.
% \fixit{PENDING
% We also generate lattice electronic Hamiltonians from 2x2 to 11x11 to test each approach's capability for benchmarks with different sizes.}

\begin{table}[htbp]
\caption{UCCSD ansatz properties by molecule}
\label{tab:uccsd}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Molecule} & \textbf{Orbitals} & \textbf{Particles} & \textbf{Qubits} & \textbf{\# 1stExc.} & \textbf{\# 2ndExc.} \\
\hline
LiH        & 6  & (2,2)   & 12 & 32   & 152     \\
BeH$_2$    & 7  & (3,3)   & 14 & 48   & 360     \\
CH$_4$     & 9  & (5,5)   & 18 & 80   & 1040    \\
MgH$_2$    & 11 & (7,7)   & 22 & 112  & 2072    \\
SiH$_4$    & 13 & (9,9)   & 26 & 144  & 3456    \\
CO$_2$     & 15 & (11,11) & 30 & 176  & 5192    \\
CH$_3$Cl   & 17 & (13,13) & 34 & 208  & 7280    \\
C$_2$F$_2$ & 20 & (15,15) & 40 & 300  & 15450   \\
H$_4$Si$_2$& 22 & (16,16) & 44 & 384  & 25632   \\
C$_2$H$_4$F$_2$ & 24 & (17,17) & 48 & 476 & 39746 \\
CH$_3$ClS  & 26 & (21,21) & 52 & 420  & 30450   \\
COCl$_2$   & 28 & (24,24) & 56 & 384  & 25056   \\
C$_4$N$_2$ & 30 & (19,19) & 60 & 836  & 124982  \\
C$_3$H$_7$NO & 32 & (20,20) & 64 & 960 & 165360 \\
C$_4$H$_4$N$_2$ & 34 & (21,21) & 68 & 1092 & 214578 \\
\hline
\end{tabular}}
\end{center}

\end{table}

\Para{Hardware Architecture}
We evaluate on 3 modern quantum computing architectures: IBM heavy-hex (e.g., Boston), square grid (e.g., Miami), and a linear architecture. 
These architectures represent a spectrum of connectivity patterns in current superconducting quantum hardware, including both NISQ and Fault-tolerant quantum devices.  
For Boston and Miami, our method first extracts a linear chain that spans most of, if not all, qubits (shown in Appendix~\ref{appendix:linear-pattern}). 
We then apply our technique along this line. 
Therefore, the result of our approach gives lower bound of complexity due to unleveraged additional connectivity beyond the extracted linear chain. 
% while prior circuit synthesis frameworks exploit the full connectivity of the device. \winston{This feels a bit negative, maybe can say this restriction is a strength, as our approach gives lower bounds on the full potential of this technique. Perhaps future work could focus on capitalizing on connectivity.}

\Para{Metrics} 
We evaluate the hardware compilation process of all approaches over three metrics: total gate count, circuit depth, and compilation time.
Total gate count and circuit depth represent the resource cost and critical path length for a hardware circuit.
SWAP gates are decomposed into 3 CNOT gates prior to recording these two metrics.
Compilation time is the duration required for one approach to compile a set of Pauli strings to a hardware circuit.
This excludes time needed to construct the Hamiltonian and Pauli strings, as well as circuit postprocessing shared amongst all approaches.
These metrics are commonly used in various quantum circuit compilers~\cite{linearqft, li+:asplos19,molavi+:micro22,zhang+:asplos21}.

\Para{Baselines}
We evaluate against JW and BK, as they represent high and low Pauli weight mappings, respectively.
HATT and Fermihedral offer lower Pauli weight, but are orthogonal to our focus on regularity in Pauli strings.
We compare against Tetris and Paulihedral compilers, as they are representative state-of-the-art hardware compilers for VQE workloads.
In total, we have four baseline combinations of: Paulihedral+JW, Paulihedral+BK, Tetris+JW, and Tetris+BK.
Finally, we apply a targeted post-processing pass to all compilers: self-inverse gate cancellation, single-qubit gate merging, and SWAP decomposition into CNOTs.

\Para{Setup}
All experiments were run on an HPC compute cluster with varying Intel CPU models (e.g., Intel(R) Xeon(R) Platinum 8358 CPU @ 2.60GHz, Intel(R) Xeon(R) Gold 6230R CPU @ 2.10GHz) and operating systems (e.g., Red Hat Enterprise Linux 9 and CentOS Linux 7). 
Tetris's default setting uses a lookahead step which causes runtime to exceed the cluster's 72-hour timeout.
We disable lookahead for the 3 largest UCCSD molecules, along with the all-to-all hamiltonians to ensure complete coverage across all benchmarks.

\vspace{-0.1in}
\subsection{Q1: Reduction in Gate Count and Circuit Depth}
\label{sec:q1}
We compare gate count and circuit depth for the UCCSD benchmark because they are important to determine the execution performance in both NISQ and fault-tolerant quantum devices. 
Since there is no one baseline approach that is better than all others, we compare the improvement of \sysname{} relative to the best baseline's output for each benchmark.

\Para{Total Gate Count}
CNOT gates dominate the total gate count and are \sysname{}'s primary optimization target.
\sysname{} reduces CNOT count by $58.27\%$ (Linear), $53.97\%$ (Boston), and $27.27\%$ (Miami) (Figure~\ref{fig:total}). 
Improvement is strongest on linear and decreases with increased connectivity, as \sysname{}'s linear chain approach does not take advantage of increased connectivity.
This translates to total gate count reduction of $48.59\%$ (Linear), $43.01\%$ (Boston), and $11.57\%$ (Miami) (Figure~\ref{fig:total}).
Overall, we observe \sysname{} consistently outperforms all approaches on Linear and Boston, while remaining competitive with the best of all baselines (which is different across benchmarks) on Miami. 

Note that some CNOT gates are generated from SWAP (breakdown in Appendix~\ref{appendix:figures}). 
\sysname{} tends to utilize more SWAPs than other compilers. 
This is because \sysname{} performs qubit reordering to establish a favorable mapping using SWAP gates before circuit execution. 
Such a reordering aligns qubits involved in subsequent operations, enabling more effective gate cancellation in later steps.
Although \sysname{} incurs additional SWAP overhead, it achieves a lower overall CNOT count, making this tradeoff beneficial.


\begin{figure*}[t]
\centerline{\includegraphics[width=\textwidth]{EvaluationFigures/total.png}}
\vspace{-0.1in}
\caption{Total gate count comparison on different molecules and architectures (\sysname{} normalized to 1.0). CNOT gate count is overlaid, with further breakdown in Appendix~\ref{appendix:figures}.}
\label{fig:total}
\end{figure*}

\begin{figure*}[t]
\centerline{\includegraphics[width=\textwidth]{EvaluationFigures/depth.png}}
\vspace{-0.1in}
\caption{Circuit depth comparison on different molecules and architectures (\sysname{} normalized to 1.0).}
\label{fig:depth}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{EvaluationFigures/complete_n4.png}
    \vspace{-0.1in}
    \caption{Total gate count and depth normalized to $N^4$ for all-to-all Hamiltonians on Boston.}
    \label{fig:complete_n4}
\end{figure}




\begin{table}[tbp]
\caption{Gate count breakdown for Tetris (TET), Paulihedral (PH), and \sysname{}, using Jordan-Wigner (JW) and Bravyi-Kitaev (BK), across different hardware topologies, compiling UCCSD ansatz for C\textsubscript{4}H\textsubscript{4}N\textsubscript{2} (68 qubits). 
\textsc{\sysname{}} produces identical results across all architectures.} 
\label{tab:gate_count}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|r|r|r|}
\hline
\textbf{Arch} & \textbf{Compiler} & \textbf{CNOT} & \textbf{Clifford 1Q} & \textbf{RZ} \\
\hline
\multirow{5}{*}{Linear} & \textsc{Tet}+JW & 42,603,032 & 2,261,252 & 859,404 \\
 & \textsc{Tet}+BK & 50,784,442 & 3,749,976 & 859,404 \\
 & \textsc{PH}+JW & 40,875,374 & 1,759,089 & 859,404 \\
 & \textsc{PH}+BK & 52,964,865 & 2,134,139 & 859,404 \\
 & \textsc{\sysname{}} & 7,703,178 & 2,577,910 & 859,404 \\
\hline
\multirow{5}{*}{Boston} & \textsc{Tet}+JW & 52,825,960 & 3,213,168 & 859,404 \\
 & \textsc{Tet}+BK & 34,749,240 & 4,217,391 & 859,404 \\
 & \textsc{PH}+JW & 23,311,396 & 1,285,155 & 859,404 \\
 & \textsc{PH}+BK & 23,847,989 & 2,002,719 & 859,404 \\
 & \textsc{\sysname{}} & 7,703,178 & 2,577,910 & 859,404 \\
\hline
\multirow{5}{*}{Miami} & \textsc{Tet}+JW & 25,663,888 & 2,168,896 & 859,404 \\
 & \textsc{Tet}+BK & 26,265,837 & 3,321,044 & 859,404 \\
 & \textsc{PH}+JW & 11,152,927 & 613,090 & 859,404 \\
 & \textsc{PH}+BK & 14,468,396 & 1,240,679 & 859,404 \\
 & \textsc{\sysname{}} & 7,703,178 & 2,577,910 & 859,404 \\
\hline
\end{tabular}
}

\end{table}

\begin{table*}[htbp]
\centering
\caption{Compiler runtime, where Improv. is (best baseline - \sysname{}) / best baseline.}
\label{tab:runtime_comparison}
\vspace{-0.1in}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|l|l|r|rr|rr|rr|rr|}
\hline
\multirow{2}{*}{\textbf{Arch}} &\multirow{2}{*}{\textbf{Problem}} &\multicolumn{9}{c|}{\textbf{Runtime (s)}} \\
\cline{3-11}
 & & \textbf{\sysname{}} & \multicolumn{2}{c|}{\textbf{Paulihedral+BK}} & \multicolumn{2}{c|}{\textbf{Paulihedral+JW}} & \multicolumn{2}{c|}{\textbf{Tetris+BK}} & \multicolumn{2}{c|}{\textbf{Tetris+JW}} \\
\cline{4-5}\cline{6-7}\cline{8-9}\cline{10-11}
 & & & \textbf{Time (s)} & \textbf{Improv.} & \textbf{Time (s)} & \textbf{Improv.} & \textbf{Time (s)} & \textbf{Improv.} & \textbf{Time (s)} & \textbf{Improv.} \\
\hline
\multirow{5}{*}{MIAMI} & UCCSD MgH2 & 0.8 & 4.4 & $-$80.6\% & 3.8 & $-$77.9\% & 63.6 & $-$98.7\% & 62.7 & $-$98.6\% \\
 & UCCSD C2F2 & 9.2 & 29.4 & $-$68.6\% & 74.3 & $-$87.6\% & 6590.1 & $-$99.9\% & 4241.3 & $-$99.8\% \\
 & UCCSD C2H4F2 & 26.7 & 73.4 & $-$63.7\% & 251.6 & $-$89.4\% & 30359.5 & $-$99.9\% & 31434.2 & $-$99.9\% \\
 & Full Rank $n=40$ & 110.5 & 280.0 & $-$60.6\% & 772.3 & $-$85.7\% & 249.7^* & $-$55.8\% & 300.6^* & $-$63.3\% \\
 & UCCSD C4H4N2 & 188.4 & 446.1 & $-$57.8\% & 3643.6 & $-$94.8\% & 353.4^* & $-$46.7\% & 709.6^* & $-$73.5\% \\
\hline
\multirow{5}{*}{BOSTON} & UCCSD MgH2 & 0.8 & 4.6 & $-$81.5\% & 5.1 & $-$83.4\% & 64.2 & $-$98.7\% & 63.2 & $-$98.7\% \\
 & UCCSD C2F2 & 9.3 & 23.7 & $-$61.0\% & 64.8 & $-$85.7\% & 6543.5 & $-$99.9\% & 4242.3 & $-$99.8\% \\
 & UCCSD C2H4F2 & 26.3 & 59.8 & $-$56.1\% & 142.5 & $-$81.6\% & 30234.3 & $-$99.9\% & 31531.4 & $-$99.9\% \\
 & Full Rank $n=40$ & 108.0 & 229.4 & $-$52.9\% & 472.1 & $-$77.1\% & 256.9^* & $-$58.0\% & 311.3^* & $-$65.3\% \\
 & UCCSD C4H4N2 & 188.1 & 394.9 & $-$52.4\% & 1516.3 & $-$87.6\% & 400.3^* & $-$53.0\% & 588.2^* & $-$68.0\% \\
\hline
\multirow{5}{*}{LINEAR} & UCCSD MgH2 & 0.9 & 3.1 & $-$72.0\% & 3.6 & $-$76.1\% & 62.1 & $-$98.6\% & 61.1 & $-$98.6\% \\
 & UCCSD C2F2 & 9.2 & 21.7 & $-$57.7\% & 43.8 & $-$79.1\% & 4471.7 & $-$99.8\% & 4203.0 & $-$99.8\% \\
 & UCCSD C2H4F2 & 26.6 & 61.5 & $-$56.7\% & 137.6 & $-$80.6\% & 30234.9 & $-$99.9\% & 31509.0 & $-$99.9\% \\
 & Full Rank $n=40$ & 106.9 & 239.0 & $-$55.3\% & 463.4 & $-$76.9\% & 255.8^* & $-$58.2\% & 280.3^* & $-$61.9\% \\
 & UCCSD C4H4N2 & 188.5 & 584.5 & $-$67.8\% & 2243.0 & $-$91.6\% & 587.6^* & $-$67.9\% & 801.2^* & $-$76.5\% \\
\hline
\multicolumn{11}{r}{$^*$Lookahead disabled for Tetris.}
\end{tabular}
}
\end{table*}

\Para{Single-Qubit Gates}
\sysname{} introduces more single-qubit gates than baselines (Table~\ref{tab:gate_count}). 
This is because of an inherent tradeoff of our approach: Tetris and Paulihedral freely reorder strings across excitation terms to maximize the single-qubit cancellation, while \sysname{} fixes execution order within excitation term groups to enable more CNOT cancellation. 
Additionally, our SWAP-based remapping between atomic groups explores more CNOT gate cancellation opportunities at the cost of fewer single-qubit cancellations.
Fortunately, the increased single-qubit gates usage in our approach is all from Clifford gates, while non-Clifford gates usage (e.g., \# RZ gates) remain unchanged. 
Recent advances in magic state cultivation~\cite{chen2026efficient, gidney2024magic} show that in fault-tolerant quantum computing, the non-clifford gate (T) cost is on par with two-qubit Clifford gates (CNOT). 
This shift makes optimization of CNOT and T gates equally crucial. 
More importantly, as Figure~\ref{fig:total} shows, 1-qubit Clifford gates constitute a small fraction of total gate count; our approach can ultimately benefit the overall performance in gate count. 
% (\fixit{REF algorithm}).

% However, additional Clifford single-qubit gates relative to baselines , though these constitute a fraction of total gate count and are cheaper than CNOTS on both NISQ and fault-tolerant devices [\fixit{CITATION NEEDED}].

\Para{Circuit Depth}
We measure the circuit depth output by different compilers for various quantum hardware topologies (e.g., Linear, Boston and Miami). 
Smaller circuit depth means a more efficient execution result. 
\sysname{} reduces circuit depth by $47.53\%$ on Linear and $32.59\%$ on Boston. 
Moreover, as the complexity of the molecular benchmarks increases, the performance gap between \sysname{} and prior compilers continues to widen. 
Additionally, as the connectivity of the target architecture increases, the advantage of \sysname{} becomes less pronounced. For example, the performance margin on the Miami architecture is smaller than that on Boston. 
On Miami, \sysname{} shows comparable performance with the best of baselines. 
For some benchmarks such as C4N2, \sysname{} trails behind the best baseline by $14.06\%$ mainly because our approach first maps the hardware topology to a linear structure, thereby not fully exploiting the additional connectivity available in the architecture, 
which may limit certain optimization opportunities. 
Leveraging these connectivities in architecture to further optimize Accordion's performance circuit depth is left for future improvement. But note that, when considering both gate count and depth in terms of quantum volume, Accordion is the best for all cases.
% , even in the most restricted linear connectivity. 






\begin{mdframed}[linewidth=0.8pt, innerleftmargin=6pt, innerrightmargin=6pt]
\textbf{Q1 Summary} \sysname{}'s compilation output gives a smaller circuit depth than other approaches for all architectures.
The benefit is particularly visible on architectures with limited connectivity. 
\end{mdframed}

% \paragraph{Lattice}
% \fixit{PENDING}


\subsection{Q2: Scaling Capability}
We analyze how our approach scales when we increase the size of the problem. 
To test scalability, we create all-to-all Hamiltonians with various numbers of qubits because the number of its second excitation terms increases proportionally to \# qubits. 
This is not obvious for the benchmarks listed in Table~\ref{tab:uccsd} because some molecules have relatively sparse excitation terms. 
We report results on Boston as a representative real hardware architecture. 
% \winston{mention gate depth is derivative metric of gate count}

For the $N$ qubit all-to-all Hamiltonian, the number of second excitation terms grows as $\binom N4=O(N^4)$. 
Results discussed in \textsection\ref{sec:q1} have shown that at least $\binom N4$ RZ gates are required for all approaches, so we need at least $\Omega(N^4)$ gate count to complete the compilation. 
For small-size problems, our method is not always optimal. 
However, as the number of qubits increases, our approach demonstrates clear advantages. 
Figure~\ref{fig:complete_n4} plots total gate count and depth normalized by $N^4$, which converges to a constant for \sysname{} while other baselines grow superquartically. 
This benefit is particularly important given the long-term trend toward large-scale quantum computing.

\vspace{0.05in}
\begin{mdframed}[linewidth=0.8pt, innerleftmargin=6pt, innerrightmargin=6pt]
\textbf{Q2 Summary} Compared with baselines, \sysname{}'s compilation result is more scalable in terms of both gate count and circuit depth as the problem size increases. 
\end{mdframed}



\subsection{Q3: Compilation Time}
We record the compilation time of compiling the hardware circuit for all approaches. 
This metric determines how long users have to wait to get results. 
A sample of representative benchmarks across various sizes is displayed in Table~\ref{tab:runtime_comparison}.

\sysname{} completes all benchmarks within 200 seconds and is always able to outperform the baseline compilation time by  $36.89\%\verb|-|99.94\%$ across all benchmarks.
We note that even when we disable lookahead for Tetris (which speeds up the compilation time of Tetris at the cost of more gate count usage), we still have a faster speed. 
For complex molecules such as C2H4F2, it takes around 8.7h for Tetris to complete, while \sysname{} completes in 26s.
Furthermore, for any fixed problem and compiler, changing the architecture can give drastically different runtimes (e.g., 3643s in Miami vs 1516s in Boston for Paulihedral+JW to finish compilation for C4H4N2). 
In contrast, our approach has a consistent compilation time across this parameter.
This result is due to Paulihedral and Tetris relying on architecture-dependent heuristics, whereas \sysname{} has a deterministic algorithm by treating all of them as a linear architecture.
\vspace{0.05in}
\begin{mdframed}[linewidth=0.8pt, innerleftmargin=6pt, innerrightmargin=6pt]
\textbf{Q3 Summary} \sysname{} is able to get the circuit synthesis result several orders of magnitude faster (e.g., from hours to seconds) with a consistent performance across different architectures.
\end{mdframed}




==> MaterialScience.tex <==
% \subsection{Lattice Hamiltonian}
% \label{sec:materialscience}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{Figures/grid.pdf}
%     \vspace{-0.1in}
%     \caption{Hamiltonians in material science: Particles are arranged on a m$\times$n grid, where interactions are only between particles connected by \textcolor{red}{horizontal edges} or \textcolor{blue}{vertical edges}.
%     % \winston{Maybe call these particles or objects instead of qubits. Qubits are supposed to model something, a bit confusing here, since it looks like we assume grid connectivity.}
%     }
%     \label{fig:grid}
% \end{figure}

% In applications such as material science, the fermionic Hamiltonian is defined over a lattice structure. 
% As is shown in equation~\ref{eq:materialscience-hamiltonian}, interactions are restricted to pairs of orbitals that correspond to adjacent sites on a 2D grid.

% If we consider a lattice with $m$ rows, $n$ columns, and $N = m \times n$ qubits (shown in Figure~\ref{fig:grid}). 
% Indices $(0,1,2,3)$ form a valid combination 
% % since both $(0,1)$ and $(2,3)$ correspond to adjacent sites. 
% but $(0,1,2,4)$ is invalid because $(2,4)$ does not correspond to an edge. 
% More formally, for any valid combination $(p, q, r, s)$, let $e_1 = (p, q)$ and $e_2 = (r, s)$ denote two edges in the lattice. 
% Then, they must follow the condition $(p + 1 = q \;\text{or}\; p + n = q) \quad \text{and} \quad (r + 1 = s \;\text{or}\; r + n = s)$. 
% The number of valid terms in the Hamiltonian is $O(N^2)$. 
% For simplicity, we assume $m = n = \sqrt{N}$ in the following.

% \begin{equation}
% H = \sum_{(i,j)\in E} a_i^\dagger a_j + \sum_{(i,j)\in E}\;\sum_{(k,\ell)\in E} a_i^\dagger a_j^\dagger a_k a_\ell
% \label{eq:materialscience-hamiltonian}
% \end{equation}

% % \subsection{Term on edges only}
% \subsubsection{Overall scheduling algorithm}
% \begin{algorithm}[t]
% \caption{Hierarchical Schedule for lattice hamiltonians}
% \label{algo:lattice-synthesis}
% \begin{algorithmic}[1]

% \For{each edge $e_2$ = (r,s) in the grid}
%     \If {$e_2$ is a horizontal edge}
%         \State // Schedule RR terms
%         \For{p = 0; p + 1 < s; p++}
%         \State Execute the term with $e_1$=(p, p+1) and $e_2$
%         \EndFor 
%         \State // Schedule CR terms
%         \For{p = 0; p + n < s; p++}
%         \State Execute the term with $e_1$=(p, p+n) and $e_2$
%         \EndFor 
%     \ElsIf {$e_2$ is a vertical edge}
%         \State // Schedule RC terms
%         \For{p = 0; p + 1 < s; p++}
%         \State Execute the term with $e_1$=(p, p+1) and $e_2$
%         \EndFor 
%         \State // Schedule CC terms
%         \For{p = 0; p + n < s; p++}
%         \State Execute the term with $e_1$=(p, p+n) and $e_2$
%         \EndFor 
%     \EndIf
% \EndFor

% \end{algorithmic}
% \end{algorithm}

% We classify second excitation terms based on the orientations of the two involved edges. 
% Based on the direction of $e_1=(p,q)$ and $e_2=(r,s)$, we divide them into 4 types: RR for 2 horizontal edges, CR for vertical $e_1$ and horizontal $e_2$, RC for horizontal $e_1$ and vertical $e_2$, and CC for 2 vertical edges. Without loss of generality, we assume that $q < s$. 
% Algorithm~\ref{algo:lattice-synthesis} shows the concrete steps to schedule RR, CR, RC, and CC in sequence.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{Figures/Lattice.pdf}
%     \vspace{-0.1in}
%     \caption{Change the qubit mapping transition between terms for (a) RR, (b) CR, (c) RC, and (d) CC scenarios.}
%     \label{fig:Lattice}
% \end{figure}

% \Para{Initial mapping and iterative update}
% Given $e_1=(p,q)$ and $e_2=(r,s)$, the logical order is $I_{1}A_{1}Z_1A_{2}I_{2}A_{3}Z_2A_{4}I_{3}$ where positions p, q, r, s are occupied by `A'. 
% To execute it, we first of all turn them into the physical qubit order $I_{1}A_{1}A_{2}A_{3}A_{4}Z_{1}Z_{2}I_{2}I_{3}$. 
% After execution, we fix $e_2$ and update $e_1$ from $(p,q)$ to $e_1'=(p+1, q+1)$ to do the next execution. 

% \Para{Scheduling for RR terms}
% Since $p+1=q$ and $r+1=s$ in this scenario, there is no Z gate in the qubit pauli string and the initial mapping is $I_{1}A_{1}A_{2}A_{3}A_{4}I_{2}I_{3}$. 
% When changing $e_1$ from (p,q) to (p+1, q+1), the first member of $I_2$ becomes A and $A_1$ becomes I. 
% As is shown in Figure~\ref{fig:Lattice}(a), we need 2 SWAPS to move the first member of $I_2$ to the position after $A_{2}$ to realize the target physical mapping of $(e_1', e_2)$ term.

% \Para{Scheduling for CR terms}
% Since $p+n=q$ and $r+1=s$ in this scenario, there only exists $Z_{1}$ whose length is $n$ and the initial physical mapping becomes 
% $I_{1}A_{1}A_{2}A_{3}A_{4}Z_{1}I_{2}I_{3}$. 
% When changing $e_1$ from (p,q) to (p+1, q+1), the first member of $Z_1$ becomes A, the first member of $I_2$ becomes A while and $A_2$ becomes Z. 
% Therefore, Figure~\ref{fig:Lattice}(b) shows all movements required to reach the target physical mapping of $(e_1', e_2)$, including moving A's forward to the position after $A_1$ and moving Z backward to the position after $Z_1$. 


% \Para{Scheduling for RC terms}
% Since $p+n=q$ and $r+1=s$ in this scenario, $Z_1$ is empty and $Z_{2}$'s length is $n$. 
% The initial physical mapping becomes $I_{1}A_{1}A_{2}A_{3}A_{4}Z_{1}I_{2}I_{3}$. 
% When changing $e_1$ from (p,q) to (p+1, q+1), the first member of $I_2$ becomes A, so Figure~\ref{fig:Lattice}(c) that we should move that member to the position after $A_2$. 

% \Para{Scheduling for CC terms} 
% Since $p+n=q$ and $r+n=s$ in this scenario, both $Z_1$'s and $Z_{2}$'s length are $n$ and
% the initial physical mapping is $I_{1}A_{1}A_{2}A_{3}A_{4}Z_{1}Z_{2}I_{2}I_{3}$. 
% % \winston{Missing $Z_2$}
% When changing $e_1$ from (p,q) to (p+1, q+1), the first member of $Z_1$ and $I_2$ become A, and $A_2$ becomes $Z$. 
% Figure~\ref{fig:Lattice}(d) shows that we should move As in $Z_1$ and $I_2$ to the position before $A_3$ and move Z to the position after $Z_1$. 

% \Para{Scheduling for terms where q > r.} When doing the scheduling for RC, CC terms, there might be some terms where q is larger than r, meaning that the position of $A_2$ is larger than that of $A_3$. 
% However, for each vertical edge, there are at most $\sqrt{N}$ terms whose q has larger value than r and changing from one term to another takes at most $N$ steps. 
% The total complexity for these terms is at most $N*N*\sqrt{N}=O(N^{2.5})$.

% \subsubsection{Complexity analysis}
% Each iteration of RR scheduling takes 2 SWAPs while each iteration of others (CR, RC, and CC) takes $\sqrt{N}$ SWAPs because of the length of $Z_1$ and $Z_2$.
% There are $O(N)$ possible edges $e_2=(r,s)$ on the grid, so the overall complexity is $O(N^{2.5})$.



% \xiangyu{state transition from horizontal to vertical takes N steps}

==> approach.tex <==
\section{Accordion Implementation}
\label{approach}
This section presents our end-to-end compilation approach for electronic Hamiltonians to generate quantum circuits from fermionic operators. 
We fix JW mapping and design specialized circuit synthesis techniques 
tailored to the resulting Pauli operators, targeting architectures with linear connectivity. 
Our approach considers the representative class of Hamiltonians, all-to-all Hamiltonians. 
We first divide Pauli strings into groups (\textsection\ref{sec:pauligroup}) and present algorithms to do intra (\textsection\ref{sec:intra-atomic}) and inter (\textsection\ref{sec:inter-atomic}) group scheduling. 
% that are applicable to both classes of Hamiltonians (\textsection\ref{sec:common}), and then present unique ones tailored to each class.

Electronic Hamiltonians consist of two types of terms: the first excitation term ($\sum_{p,q} h_{pq}\,a_p^\dagger a_q$) and the second excitation term ($\tfrac12\sum_{p,q,r,s} h_{pqrs}\,a_p^\dagger a_q^\dagger a_r a_s$). 
The dominant compilation cost arises from implementing Pauli strings corresponding to the second excitation term due to its complexity. 
% While the first excitation term gives rise to $O(N^2)$ Pauli strings under JW mapping, 
% The second excitation term dominates the overall compilation complexity 
% leads to $O(N^4)$ Pauli strings due to all combinations of $0 \leq p < q < r < s < N$, 
% and thus . 
Therefore, we focus on the efficient implementation of Pauli strings corresponding to the second excitation term in this section. 
The exact form of this Pauli string can be described by the pattern $I^*AZ^*AI^*AZ^*AI^*$, where * quantifies 0 or more copies and $A$ is replaced with $X$ or $Y$ such that the string has an odd number of $X$s and $Y$s.
This is explicitly written in Equation~\ref{eq:jw-pauli}, from Appendix A of \citet{uccsd}.
The techniques developed can be applicable to the first excitation term as well. 
Evaluation (\textsection\ref{sec:eval}) demonstrates that they remain effective for practical chemistry instances, where not all Hamiltonian terms exist.

\begin{align}
\label{eq:jw-pauli}
&\bigotimes_{b=l+1}^{k-1}Z_b
\bigotimes_{a=j+1}^{i-1}Z_a
(X_lX_jY_kX_i
+Y_lX_kY_jY_i
+X_lY_kY_jY_i\\
+&X_lX_kX_jY_i
-Y_lX_kX_jX_i
-X_lY_kX_jX_i
-Y_lY_kY_jX_i
-Y_lY_kX_jY_i)
\nonumber\\
=&\sum_{
\substack{
A_l,A_k,A_j,A_i\in\{X,Y\}
\\
\text{\#X and Y both odd}
}}
\pm
I_1\ldots I_{l-1}
\otimes A_l\otimes
Z_{l+1}\ldots Z_{k-1}
\otimes A_k
\nonumber\\
&\otimes
I_{k+1}\ldots I_{j-1}
\otimes A_j\otimes
Z_{j+1}\ldots Z_{i-1}
\otimes A_i\otimes
I_{i+1}\ldots I_n
\nonumber
\end{align}
% where not all Hamiltonian terms exist.

% Although our methods are developed for general electronic Hamiltonians, 
% evaluation (\textsection\ref{sec:eval}) demonstrates that they remain effective for practical chemistry instances, 
% where not all Hamiltonian terms exist.



% Accordingly, this section includes examples and algorithms focusing on the efficient implementation of Pauli strings belonging to the second excitation term. 


\begin{table*}[]
\renewcommand{\arraystretch}{1.5}
\caption{Divide all Pauli Strings into various groups. `A' can represent either the `X' gate or the `Y' gate. We show the group size assuming the total number of qubits is N. pos(...) is a function that returns the index of a particular character. $\binom{m}{n}$ represents combinations to calculate the number of ways to choose a subset of n items from m distinct items.}
\label{table:GroupDef}
\resizebox{\linewidth}{!}{
\begin{tabular}{llccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Definition}}                          & \multicolumn{1}{c}{\textbf{\# groups}} & \multicolumn{1}{c}{\textbf{\# terms per group}} & \multicolumn{1}{c}{\textbf{Example}} \\ \midrule
\textbf{Singleton Group}           & Same position for \textbf{the 1st, the 2nd, the 3rd, and the 4th} operator (`X' or `Y') & $\binom{N}{4}*8$ & 1 & \{"XXIXY"\}          \\ 
\textbf{Atomic Group}           & Same position for \textbf{the 1st, the 2nd, the 3rd, and the 4th} `A'  & $\binom{N}{4}$ & 8 & \{"XXIXY", "XYIYY", ...\}\\ 
\textbf{Mini Group}             & Same position for \textbf{the 1st, the 3rd, and the 4th} `A'          & $\binom{N}{3}$ & pos(3rd 'A') - pos(1st 'A') - 1 & \{"AAIAA", "AZAAA", ...\}          \\ 
\textbf{Medium Group} & Same position for \textbf{the 1st and the 4th} `A'  & $\binom{N}{2}$ & $\binom{pos(4th 'A') - pos(1st 'A') - 1}{2}$ & \{"AZAAA", "AAAZA", ...\} \\ 
\textbf{Large Group}  & Same position for \textbf{the 1st} `A' ONLY        & $\binom{N}{1}$ & $\binom{N - 2 - pos(1st 'A')}{3}$ & \{"AZAAA", "AAAAI", ...\} \\ \bottomrule
\end{tabular}}
\end{table*}

\subsection{Pauli string grouping}
\label{sec:pauligroup}
% One benefit of choosing the JW mapping is that its output Pauli strings contain structural patterns. 
% We observe that many of these strings share common components, such as identical positions of non-identity operators or consistent relative ordering among them. 
We put strings with similar patterns into the following groups according to the positions of their non-identity operators (denoted as `A' $\in$ \{`X', `Y'\}). 

\textbf{Singleton Group} contains strings where all 4 non-identity operators appear at the same set of positions.
 \textbf{Atomic Group} has strings whose all four `A' operators' position are fixed.
\textbf{Mini Group} consists of strings with common positions of the 1st, 3rd, and 4th `A' operators, varying the 2nd `A' operator within a range.
\textbf{Medium Group} contains strings with only the positions of the 1st and 4th `A' operators fixed.
\textbf{Large Group} includes strings with the position of only the 1st `A' operator fixed.
Other details are shown in Table~\ref{table:GroupDef}. 
% (shown in ). 
% To be specific, our strategy clusters Pauli strings according to the positions of their non-identity operators (denoted as `A' $\in$ \{`X', `Y'\}) into the following groups.


% \subsection{Common strategy}
% \label{sec:common}
% We describe strategies that can be shared by all-to-all and lattice Hamiltonians. 

\subsection{Intra group scheduling}
\label{sec:intra-atomic}
There is only one term per Singleton Group, so no intra-group scheduling is required for that group. 
We focus on the intra-group scheduling for the Atomic Group and the Mini Group. 
The intra-group scheduling for the Medium Group and the Large Group is identical to the inter-group scheduling for the Mini Group.

\Para{Intra atomic group scheduling}
To execute one Pauli string within an atomic group, we select one of the `X'/`Y' operators as the root node and construct a connectivity path that links all qubits to this root via a sequence of CNOT gates to implement the exponentiation of the Pauli string. A naive execution order (Figure~\ref{fig:GroupGate}(a)) follows the original qubit layout. 
Since the qubits corresponding to the 2nd and 3rd 
`X'/`Y' operators are often separated by a sequence of identity (`I') operators; the established connectivity path incurs multiple SWAP operations to move qubits across these inactive regions. 
When the number of `I' operators is large, this leads to a significant overhead. 
Further, since each atomic group contains 8 Pauli strings with identical positional patterns, this SWAP overhead is incurred in every string in the group. 

To mitigate this issue, we propose \textit{qubit remapping} at the beginning of the group execution. 
Concretely, we reorder the qubits such that those corresponding to 
`X'/`Y', `Z', and `I' operators are placed into contiguous regions (Figure~\ref{fig:OrderWithinAtomicGroup}(b)). 
By clustering operators together, we ensure that all required CNOT connections can be realized without additional SWAP operations during the execution of individual Pauli strings. 
% This effectively eliminates repeated SWAP overhead and reduces circuit complexity.

In addition, this strategy enables gate cancellation across Pauli strings within the same atomic group. 
As illustrated in Figure~\ref{fig:OrderWithinAtomicGroup}, when executing two Pauli strings sequentially, the common subpath from the leaf nodes to the root induces identical sequences of CNOT, as well as basis transformation gates (H and S).
By aligning the execution order of Pauli strings, these overlapping gate sequences can be directly canceled, resulting in a reduction of O(N) gates per transition.

Therefore, we schedule Pauli strings such that consecutive strings share the longest possible common suffix. 
For example, assuming the 1st non-identity operator is chosen as the root, XX\fixit{YXZZI} and YY\fixit{YXZZI} share a long common suffix \fixit{YXZZI}, leading to more gate cancellation in execution.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{Figures/GroupGate.pdf}
    \vspace{-0.1in}
    \caption{(a) is a naive approach; (b) is our solution to save SWAP gates by putting X/Y gates adjacent to each other, clustering Z gates and I gates together respectively.} 
    % \winston{Same as Figure {\ref{fig:OrderWithinAtomicGroup}}}\xiangyu{I agree with Winston that they share a lot of similarity. The gist here I want to show is that it is worthwhile for us to put X/Y gates adjacent to each other because this can save future SWAP gates. This is not reflected in Figure {\ref{fig:OrderWithinAtomicGroup}}}}
    \label{fig:GroupGate}
\end{figure}

% \subsection{All-to-all Hamiltonian}
% \label{sec:all-to-all}
% % \xiangyu{Mention that we have intra and inter group scheduling.}
% We list scheduling algorithms designed for all-to-all Hamiltonian. 
% We divide them into 2 main categories: intra-group scheduling and inter-group scheduling. 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{Figures/OrderWithinAtomicGroup.pdf}
    \vspace{-0.1in}
    \caption{Schedule 2 singleton groups (a) and (b) that share common leaf nodes for their physical qubits to cancel gates. All gates executed on the common part from leaf to root (Q1) can be cancelled.
    }
    \label{fig:OrderWithinAtomicGroup}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/GateCancel.pdf}
    \vspace{-0.3in}
    \caption{Cancel CX and SWAP gates between atomic groups ((a)$\to$(b)) and between mini groups ((b)$\to$(c)).}
    \label{fig:GateCancel}
\end{figure*}



\Para{Intra mini group scheduling}
Within each mini group, Pauli strings share fixed positions for the 1st, 3rd, and 4th `A' operators. We define two mini groups to be adjacent if the positions of their 2nd `A' operators differ by one (e.g., if one Pauli string is the same as the one in Table~\ref{table:PauliLogic} except putting $A_2$ in position q + 1, it is an adjacent Pauli string).

To enable efficient transitions across mini groups, we first apply a global qubit remapping such that all Pauli strings follow a canonical layout of the form $\text{I}^{*}\text{AAAAZ}^{*}\text{I}^{*}$, where all `X'/`Y' operators are clustered into a contiguous region, followed by `Z' operators, and then identity operators.

Under this canonical arrangement, transitioning between two adjacent mini groups can be implemented with a constant number of SWAP operations. As illustrated in Figure~\ref{fig:GateCancel}, shifting the position of the 2nd 
`A' operator by one only requires locally adjusting the boundary of the A-region, which can be achieved using 3 SWAP gates. 
This transformation preserves the overall 
$\text{I}^{*}\text{AAAAZ}^{*}\text{I}^{*}$ pattern, ensuring that subsequent circuit constructions remain compatible with our intra-group scheduling strategy.

This strategy also enables CNOT gate cancellation. 
As illustrated in Figure~\ref{fig:GateCancel}, we consider two cases. First, for atomic groups within the same mini group (Figure~\ref{fig:GateCancel}(a) $\to$ Figure~\ref{fig:GateCancel}(b)), all Pauli strings share identical positions except qubit operators differing only in all As' operators. 
% \fixit{The gate cancellation mechanism is described in section~\ref{sec:intra-atomic}.}
Second, for atomic groups across adjacent mini groups (Figure~\ref{fig:GateCancel}(b) $\to$ Figure~\ref{fig:GateCancel}(c)), the required three SWAP operations are confined to qubits corresponding to the $A_1$, $A_2$, $A_3$, and $A_4$
operators.
As a result, the CNOT chains acting on these unaffected qubits (where Z operators sit) remain identical and can still be largely canceled across group boundaries. 

\subsection{Inter-group scheduling}
\label{sec:inter-atomic}
Our scheduling procedure proceeds by iterating over all groups hierarchically, executing mini groups in sequence.
Each group corresponds to a specific qubit mapping, some permutation of length $N$, determined by the earliest Pauli string.
Transitioning between groups is equivalent to transforming one permutation into another.
We use parallel nearest-neighbor sort \cite{habermann1972} to realize any permutation in $O(N)$ depth with adjacent swaps, giving a uniform scheduling algorithm for all inter-group transitions.
% which can realize any permutation using only nearest-neighbor swaps in $O(N)$ depth. 
% \fixit{This provides a uniform scheduling strategy for all inter-group transitions.}

\begin{table}[t]
\caption{Logical order of all qubit gates where 4 A's are in position p, q, r, and s.}
\label{table:PauliLogic}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
Pauli Logic & $\text{I}_{1}$  & $\text{A}_{1}$ & $\text{Z}_{1}$  & $\text{A}_{2}$ & $\text{I}_{2}$  & $\text{A}_{3}$ & $\text{Z}_{2}$  & $\text{A}_{4}$ & $\text{I}_{3}$  \\ \midrule
Start       & 0   & p  & p+1 & q  & q+1 & r  & r+1 & s  & s+1 \\ 
End         & p-1 & p  & q-1 & q  & r-1 & r  & s-1 & s  & n-1 \\ \bottomrule
\end{tabular}}
\end{table}


% \begin{table}[t]
% \caption{Logical order of all qubit gates where 4 A's are in position p, q+1, r, and s.}
% \label{table:PauliLogic2}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lccccccccc}
% \toprule
% Pauli Logic & $\text{I}_{1}$  & $\text{A}_{1}$ & $\text{Z}_{1}$  & $\text{A}_{2}$ & $\text{I}_{2}$  & $\text{A}_{3}$ & $\text{Z}_{2}$  & $\text{A}_{4}$ & $\text{I}_{3}$  \\  \midrule
% Start       & 0   & p  & p+1 & q+1 & q+2 & r  & r+1 & s  & s+1 \\ 
% End         & p-1 & p  & q   & q+1 & r-1 & r  & s-1 & s  & n-1 \\ \bottomrule
% \end{tabular}
% }
% \end{table}

% Given a mapping represented as a permutation of $N$ qubits, we need at most $O(N)$ steps to transform it into another target permutation~\cite{odd-even-schedule}\xiangyu{TODO: Xiangyu will check it}. 
% We adopt this approach to perform this transformation across medium and large groups. 
% Intuitively, each qubit can be moved to its target position within at most $O(N)$ steps, and there are $N$ qubits in total.

% 


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.49\textwidth]{Figures/Ordering.pdf}
%     \vspace{-0.2in}
%     \caption{We pick 2 adjacent terms (A and B) within a mini group. (a) logical and physical qubit mapping for term A; (b) logical and physical qubit mapping for term B; \textcolor{blue}{$\to$} represents the qubit mapping. Starting from term A's qubit mapping, we need 3 SWAPs to turn to the satisfied initial qubit mapping in term B (in the form of $\text{I}^{*}\text{AAAA}\text{Z}^{*}\text{I}^{*}$).
%     \winston{maybe we can drop this, also Z1 and Z2 are flipped}}
%     \label{fig:Ordering}
% \end{figure}


\subsection{Complexity analysis}
Algorithm~\ref{algo:all-to-all-synthesis} shows the order to schedule various defined groups. 
This algorithm provides gate count and circuit depth bounded by O($N^4$).
We provide a simplified proof for circuit depth proof below.

% \xiangyu{TO proofread}
% \subsubsection{Scheduling algorithm}
% \leavevmode

% We execute atomic groups within each mini group, iterate over all mini groups in a medium group, 
% then traverse medium groups within a large group, and finally proceed across large groups.
% Importantly, within the same medium group, switching the qubit mapping between adjacent mini groups requires only 3 SWAP operations.}

\begin{algorithm}[t]
\caption{Schedule Hierarchy for all-to-all hamiltonians}
\label{algo:all-to-all-synthesis}
\begin{algorithmic}[1]

\For{each large group $L$}
    \State Initialize mapping for $L$
    
    \For{each medium group $M \in L$}
        \State Reuse mapping to align 4th $A$
        
        \For{each mini group $m \in M$}
            \State Apply 3 SWAPs to get the $I^{*}AAAAZ^{*}I^{*}$ form
            
            \For{each atomic group $a \in m$}
                \State Cancel adjacent Clifford gates 
                \State Execute Pauli string belonging to $a$  
            \EndFor
            
        \EndFor
    \EndFor
    
\EndFor

\end{algorithmic}
\end{algorithm}

% \subsubsection{Complexity calculation}
% \leavevmode

The overall circuit depth consists of two components: intra-group and inter-group scheduling. 
% We analyze these two components separately.
For intra-mini group scheduling, atomic groups are executed sequentially. 
Transitioning between two consecutive atomic groups requires three additional stages, 
each implementing a single SWAP gate.
Our scheduling strategy's gate cancellation (Figure~\ref{fig:GateCancel}) ensures that for all atomic groups within one mini group, each group takes only $O(1)$ depth to execute its $O(1)$ CNOT gates (except the first and the last groups, which take O(N) depth, but have O(1) amortized cost).
% The transition between each mini-group incurs $O(N)$ depth from CNOTs and SWAPs, giving $O(N^4)$ amortized depth.
There are O($N^4$) atomic groups in total, and thus, the total circuit depth of intra-group scheduling is also $O(N^4)$.

For inter group scheduling, the total number of mini, medium and large groups are $\binom{N}{3}$, $\binom{N}{2}$, and $\binom{N}{1}$ respectively (Table~\ref{table:GroupDef}). It takes $O(N)$ steps to do a transformation from one permutation to another one, thus the complexity for this scheduling is $O(N^4)$.


If we sum up intra and inter group scheduling, the total complexity is still $O(N^4)$, meaning that each term only takes constant circuit depth on average. 
The number of second excitation terms dominates that of the first excitation terms, so
the overall circuit depth for implementing the all-to-all fermionic Hamiltonian is $O(N^4)$. 
A more involved charging argument gives the $O(N^4)$ gate count bound (Appendix~\ref{appendix:gate_count_bound}).
% This is done by charging $O(1)$ CNOT and SWAP gates to the inner loop, while amortizing the remaining cost.

% \fixit{This algorithm cancels O($N$) CNOT gates and introduces constant SWAP gates between 2 adjacent mini groups}, leading to the overall $O(N^4)$ complexity of total gate count. 
% A detailed proof for gate count complexity is in Appendix~\ref{appendix:gate_count_bound}.
% Additionally, we provide a more detailed proof bounding the total gate count in 

==> conclusion.tex <==
\section{Conclusion}
\label{conclusion}

We build \sysname{}, an end-to-end framework to generate quantum circuits for fermionic Hamiltonians. 
By identifying the fermion-to-qubit mapping choice in a counter-intuitive way and designing tailored circuit synthesis algorithms, \sysname{} can generate circuits with reduced gate count and circuit depth at a faster speed than state-of-the-art approaches. 
This result has shown quantitative evidence of how fermion-to-qubit mapping affects the end-to-end compilation of a Hamiltonian. 
% \winston{add a bit about future work (capitalize on connectivity, streaming compiler implementation, other ansatz)}
% \xiangyu{Typically, we do not mention future work in conclusion. So we do not need to do that.}


==> intro.tex <==
\section{Introduction}

Simulation of fermionic systems is fundamental to several domains such as quantum chemistry and condensed matter physics. 
Computing ground-state energies of molecular Hamiltonians enables applications ranging from drug discovery to materials design. 
Variational quantum eigensolvers (VQE) have emerged as a leading approach for simulating such systems on modern quantum hardware by variationally approximating the ground state of a fermionic Hamiltonian. 

Executing the VQE workloads on quantum hardware requires transforming high-level fermionic Hamiltonians into hardware-executable quantum circuits. 
This transformation involves a multi-stage compilation pipeline. 
First, we need to turn fermionic operators into sums of Pauli strings. 
Then, these Pauli operators are synthesized into logical quantum circuits, which are further compiled into physical circuits following the device's connectivity constraints.

% \textbf{State-of-the-art approaches:} 
Prior works focus on optimizations at different stages of this pipeline. 
At the encoding stage, various fermion-to-qubit mappings (e.g., Jordan–Wigner (JW)~\cite{JW}, Bravyi–Kitaev (BK)~\cite{BK}, HATT~\cite{hatt}, and Fermihedral~\cite{Fermihedral}) have been proposed to optimize specific metrics (e.g., Pauli weight). 
At the circuit synthesis stage, works such as Tetris~\cite{Tetris} and Paulihedral~\cite{Paulihedral} exploit structural similarities among Pauli strings to reduce the cost of logical and physical circuits using heuristics. 
Figure~\ref{fig:CircuitSynthWF} shows that the number of possible paths from fermionic Hamiltonians to hardware circuits is the cross product of mapping strategies and hardware compilers. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{Figures/CircuitSynthWF.png}
    \vspace{-0.3in}
    \caption{State-of-the-art approaches generate quantum circuits through several stages: \textcircled{1} map Fermion to qubit operators, and \textcircled{2} generate hardware circuits using heuristics. We apply an end-to-end framework by fixing the mapping option and designing tailored circuit generation algorithms.}
    \label{fig:CircuitSynthWF}
\end{figure}

% \textbf{Problems in the state-of-the-art:} 
However, existing approaches are limited by their stage-wise design.
On the one side, these works are largely developed in isolation. 
% For instance, mappers in the fermion-to-qubit stage optimize Pauli weight while synthesizers in the qubit-to-circuit stage optimizes the gate count and circuit depth. 
This separation leads to missing joint end-to-end optimization opportunities.
% \winston{FRAMING Qubit Mapper optimize for weight bc better circuit. Circuit synthesizers optimize for hardware (this is one goal, they do other things too). These are counterproductive goals.}
Specifically, the BK mapper in the fermion-to-qubit stage produces Pauli operators with lower Pauli weight compared to JW. Intuitively, minimizing this will give an efficient circuit. 
Empirically, these operators generated by BK may exhibit less structural similarity. 
Given that the effectiveness of follow-up circuit synthesis techniques relies on those patterns among Pauli strings, this can lead to higher overall gate count and circuit depth. 
% \winston{FRAMING Competing goals get worse as the size of the problem scales.}
On the other side, we evaluate these techniques across increasing problem sizes. Our results (Figure~\ref{fig:ScalabilityA2A}) show that all combinations exhibit scalability issues. 
Both circuit depth and gate count grow substantially faster than the number of Pauli strings. 
Additionally, it takes several hours for existing approaches to complete compilation for several large-size benchmarks. 

The ultimate goal of execution efficiency on quantum hardware is determined by metrics such as gate count and circuit depth, not intermediate metrics like Pauli weight.
% \winston{CLARITY execution or circuit depth? should be consistent with naming}. 
Therefore, we believe that optimization efforts should be focused on end-to-end circuit efficiency, rather than on isolated improvements within individual stages of the compilation pipeline. 


% \textbf{Our approach:} 
In this paper, we take a fundamentally different approach to solve this problem with an end-to-end framework called \sysname{}. 
We anchor the compilation process on a fixed fermion-to-qubit mapping and develop tailored circuit synthesis algorithms 
that generate physical circuits with much lower complexity than state-of-the-art methods.
Concretely, we start from the JW mapping, which produces Pauli operators with regular structure. 
Then, we design a tailored optimizing circuit synthesis framework for JW's output. 
Our approach incorporates qubit mapping and circuit scheduling strategies that can maximize gate cancellation and minimize the circuit depth. 
% \winston{CLARITY what does map qubits mean. qubit mapping -> fermion to qubit overloaded}
% We also generalize 
% Our approach can be applicable to support a range of hardware topologies, including linear arrays, heavy-hex architectures, and 2D lattice layouts across both NISQ and FT quantum devices.

% \textbf{Evaluation Result: \fixit{Use the template in Zihan's paper?}}
% \fixit{Add complexity results? Big O notation. Or do you think complexity is not a good contribution of our work compared with prior work, when the Hamiltonian is full rank? If you do not think it is a good contribution, you can omit it here.}
We evaluate \sysname{} on representative quantum chemistry benchmarks across both NISQ (e.g., IBM heavy-hex) and Fault Tolerant (e.g., square grid) architecture.
Results (\textsection\ref{sec:eval}) show that \sysname{} can generate results with up to $74.39\%$ (avg is $34.39\%$) smaller gate count and up to $63.64\%$ (avg is $27.24\%$) smaller circuit depth compared to the best of existing baselines. 
% \winston{CLARITY we cannot say this. we have 3 classes of problems, while current averages are heavily weighted to UCCSD (over problems in Figure~\ref{fig:depth}). Each problem has different qualities, and we need to quantify too much for this number to even be meaningful. Just talk about Boston UCCSD, -43.01\% gate count -32.59\% depth}
% \xiangyu{Check with Wisnton, report some number here. For example, max and avarage gate count saving?} 
% \winston{Max gate count savings (against best baseline): Linear($74.39\%$) Boston($56.66\%$) Miami($23.29\%$). Average included in eval section}
We also offer a formal proof for the O($N^4$) circuit depth complexity and gate count in terms of the \# qubits for all-to-all Hamiltonians (\textsection\ref{approach}). 
% and \textsection\ref{sec:materialscience}).
In terms of the compilation time, 
\sysname{} is faster with up to $95.62\%$ (avg is $63.09\%$) time saving, offering hour-to-second speedup on several benchmarks. 
% \winston{CLARITY need to qualify runtime metrics, see above, hour-to-second also doesn't say much, we have proportional gain.}
% \winston{Max/Avg runtime savings (against best baseline): Linear($72.03\%/61.15\%$) Boston($81.52\%/60.86\%$), Miami($77.86\%/61.65\%$)}

% \fixit{show numbers}
% We further evaluate our method , all showing significant improvements in scalability compared to state-of-the-art techniques.

Our contributions can be summarized as follows:
% \winston{FRAMING these points are too vague. use this (1) end-to-end/vertical optimization framing (fix JW, codesign synthesis) (2) develop string permutation + scheduling technique $O(n)$ gate cancellation
\squishlist
     \item We build \sysname{}, an end-to-end framework for compiling electronic structure fermionic Hamiltonians with \textbf{provable linear complexity} with respect to the number of double excitation terms for the first time.
     \item We show that, contrary to the conventional wisdom, the Jordan-Wigner (JW) approach, while having the worst average Pauli-weight metric compared with other approaches such as Bravyi-Kitaev (BK) and balanced ternary tree,  can actually outperform others, only if it utilizes the efficient and tailored circuit synthesis and hardware routing techniques developed in this paper. 
     
    \item We develop Pauli-string permutation and scheduling algorithms in circuit synthesis to maximize CNOT gate cancellation and reduce SWAP gate overhead with provable worst-case linear bounds. 
   
    \item We formally prove the complexity bound of circuit depth and gate count for the full rank all-to-all Hamiltonians.
    \item We compare \sysname{} against state-of-the-art approaches for the two-stage fermionic Hamiltonian compilation pipeline over modern quantum devices, showing up to 74.39\% reduction on gate count, up to 63.64\% reduction on circuit depth, and up to 95.62\% reduction in compilation time. 
    % and analyze its improvement quantitatively. 
\squishend

% Our method offers analytic and deterministic constructions, where qubit movements and gate scheduling follow structured patterns.

==> motivation.tex <==
\section{Background}
\label{background}
In this section, we introduce essential background for this paper, including Fermionic Hamiltonians and the current works on quantum circuit synthesis.
Fundamental concepts in quantum computing are covered in standard references~\cite{QCQI}. 
\subsection{The Importance of Fermionic Hamiltonians}
% \xiangyu{Ask Zirui to check accuracy later}
Fermionic Hamiltonians are a standard mathematical model for describing interacting many-body fermionic systems.
They arise in electronic structure problems in quantum chemistry~\cite{modernQChem} and in lattice models for condensed-matter physics~\cite{QTheoryManyParticle, CondensedMFT}, where the goal is often to understand the low-energy behavior of electrons. 
In many settings, the primary computational target is the ground state and the ground-state energy, since it can predict equilibrium properties of molecules and materials. 
Solving fermionic Hamiltonians is important across multiple domains, including quantum chemistry~\cite{aspuru2005simulated, cao2019quantum}, materials science~\cite{google2020hartree}, and condensed-matter physics~\cite{stanisic2022observing}.
% \winston{LOW doesn't feel very convincing}

There are several types of Fermionic Hamiltonians for various application domains of quantum simulation. 
For example, electronic structure Hamiltonians~\cite{mcquarrie2008quantum} are for molecular systems, and the Fermi–Hubbard model~\cite{CondensedMFT} is for condensed-matter physics. 
Among these, \textit{the electronic structure Hamiltonian is particularly important}, as it directly captures the many-electron problem underlying chemistry and materials science, and serves as a primary target for quantum simulation algorithms. 
Specifically, the electronic Hamiltonian can be represented in the form of Equation~(\ref{eq:elec-hamiltonian}).

\begin{equation}
H = \sum_{p,q} h_{pq}\,a_p^\dagger a_q 
\;+\;\tfrac12\sum_{p,q,r,s} h_{pqrs}\,a_p^\dagger a_q^\dagger a_r a_s
\label{eq:elec-hamiltonian}
\end{equation} 

Such a Hamiltonian structure in Equation (1) is also arguably one of the most important ansatz being highly expressible and less susceptible to barren plateaus in variational quantum solvers. To compute the ground-state energy, another common approach is the Variational Quantum Eigensolver (VQE)~\cite{peruzzo2014variational}, which formulates the problem as a variational optimization over parameterized quantum circuits to approximate the ground state. 
The concrete structure of the quantum circuit in VQE is determined by the choice of ansatz. 
Various ansatz~\cite{mcclean2016theory,tilly2022variational} have been proposed for VQE 
and \textit{the Unitary Coupled Cluster Singles and Doubles (UCCSD)~\cite{uccsd}} is one of the most widely used options and is important for solving the ground state energy problem. 
The UCCSD ansatz is constructed from fermionic excitation operators, including single excitations of the form $a_p^\dagger a_q$ (called the first excitation term)
and double excitations of the form $a_p^\dagger a_q^\dagger a_ra_s$ (called the second excitation term), whose operator structure resembles the single qubit interaction and two qubits interaction terms in the electronic Hamiltonian in Equation~(\ref{eq:elec-hamiltonian}).
% \winston{LOW writing flow issues}

For the reasons mentioned above, in this paper, we focus on the Hamiltonian form in Equation~(\ref{eq:elec-hamiltonian}) and its compilation of the circuit from start to finish. Many practical problems in chemistry and physics simulation or VQE ansatz are embodied in such a form, with the coefficients of $h_{p,q}$ and $h_{pqrs}$ varying from problem instance to problem instance. 
% Similar to equation~\ref{eq:elec-hamiltonian}, the UCCSD ansatz is constructed from excitation operators with single ($a_p^\dagger a_q $) and double ($a_p^\dagger a_q^\dagger a_r a_s$) electron excitation operators. 



% \xiangyu{importance of electronic hamiltonian}

% , which specifies how fermionic operators are translated into parameterized unitary operations.
% \xiangyu{to calculate the ground state, we need to rely on variational quantum eigensolver (VQE) to get the solution.}


\subsection{The Compilation Pipeline for Mapping a Fermionic Hamiltonian to A Physical Circuit}
Due to the exponential complexity of simulating fermionic systems on classical computers, quantum hardware provides a natural execution platform. 
Existing approaches mainly follow a 2-stage software stack to execute a fermionic Hamiltonian (shown in Figure~\ref{fig:CircuitSynthWF}).
% , from fermion operators to qubit operators and from qubit operators to circuits, respectively. 

The \textit{fermion-to-qubit} stage encodes fermionic operators into Pauli operators, representing the original Hamiltonian as a sum of Pauli strings.
At this stage, several mappers are developed (Table~\ref{tab:mapping}) to optimize Pauli weight, the number of non-identity factors in the Pauli strings.
Jordan-Wigner~\cite{JW} is the most direct mapper, producing Pauli strings with regular, predictable structure, at the cost of $O(N)$ Pauli weight.
The Bravyi-Kitaev~\cite{BK} mapper reduces Pauli weight to $O(\log(N))$ by using a tree-based encoding, at the cost of more irregular patterns.
HATT~\cite{hatt} offers a further optimization by constructing an adaptive ternary tree specific to the Hamiltonian, and Fermihedral~\cite{Fermihedral} uses a SAT solver to find the globally optimal minimal Pauli weight mapping. 
Based on our observation, the structural regularity only appears in the JW mapper's output. 


The qubit-to-circuit stage compiles these operators into quantum circuits executable on hardware. 
This typically involves decomposing exponentials of Pauli strings into sequences of quantum gates and compiling them according to the hardware architecture. 
Representative approaches, such as Tetris \cite{Tetris} and Paulihedral \cite{Paulihedral}, employ optimization techniques to reduce gate count and circuit depth. 
These methods use heuristics to capitalize on gate cancellation while minimizing SWAP based routing cost.
As a result, the compilation optimization and duration both depend on the structure of the input Pauli strings and the target architecture.
For large problems, the compilation time can grow significantly as the heuristics explore larger search spaces.

% To remedy this problem, in this paper, we develop an approach to generating physical circuits directly from the fermionic Hamiltonian in one stage.


% \xiangyu{importance of UCCSD Ansatz}


    

 % \fixit{Maybe it is okay that we emphasize this only UCCSD ansatz, as it is one of the most important ansatz for finding the ground state energy problem -- which is already significant enough. But do mention that such form is also important type of Hamiltonian simulation. Also mention other types of ansatz and provide the reference here. Narrowing it down to a specific problem is a actually a good strategy. As long as you guys do this, I will be happy.  }

% \subsection{Two Stages of the Work }
% \xiangyu{add one table to compare different mapping approaches}

\begin{table}[]
\begin{small}
\caption{Different mappings to generate Pauli Strings.}
\label{tab:mapping}
% \winston{CLARITY drop the limitation column. it's not doing anything. alt, just do this in prose, why need table}}
\end{small}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Mapping} & \textbf{Advantage} & \textbf{Limitation} \\
\midrule
JW~\cite{JW}  & Regular structure 
    & High Pauli weight \\

BK~\cite{BK}  & Low Pauli weight
    & Irregular structure \\

HATT~\cite{hatt} & Input-adaptive mapping 
     & Less regular structure\\

Fermihedral~\cite{Fermihedral} 
     & Minimum Pauli weight 
     & Limited scalability due to SAT solver \\
\bottomrule
\end{tabular}}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ccccc}
% \toprule
% \textbf{Method} & \textbf{Mapping Type} & \textbf{Pauli Weight} & \textbf{Strengths} & \textbf{Weaknesses} \\ \midrule
% JW~\cite{JW}     & Local string        & O(n)     & Simple, deterministic       \\
% BK~\cite{BK}     & Log-tree            & O(log n) & Lower Pauli weight          \\
% Parity~\cite{Parity} & Parity-based        & O(n)     & Efficient symmetry handling \\
% HATT~\cite{hatt}   & Hardware-aware tree & O(log n) & Architecture-friendly\\
% Fermihedral~\cite{Fermihedral}   &  &  & & \\
% \bottomrule
% \end{tabular}}
\end{table}

% \xiangyu{add one table to compare qubit mapping approaches}

% \begin{table}[]
% \begin{small}
% \caption{State-of-the-art compilation frameworks that synthesize physical-qubit circuits from Pauli strings produced by various fermion-to-qubit mapping methods. \fixit{Tetris, or Paulihedral, does not provide a complexity guarantee. Would it be better to show a figure that Winston prepared, where empirically we show the scaling of other approaches is super-linear to the number of terms, while ours is?}}
% \label{table:qubitgen}
% \end{small}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lllcc}
% \toprule
% \multicolumn{1}{c}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{Core Idea}} & \multicolumn{1}{c}{\textbf{Optimization Target}} & \textbf{Algorithm} & \textbf{Complexity} \\
% \midrule
% Tetris      &  &  & Heuristic     &                         \\
% Paulihedral &  &  & Heuristic     &                         \\
% Our Approach  &  &  & Deterministic & O($n^4$)\\
% \bottomrule
% \end{tabular}}
% \end{table}

\section{Motivation}
Ultimately, what the end user really cares about is the execution efficiency (e.g., gate count and circuit depth) of generated quantum circuits. 
Existing approaches divide the compilation of fermionic Hamiltonians into 2 separate stages and can lead to potential suboptimalities of the final results. 
By examining state-of-the-art compilation workflows that work in isolation, we have made several key observations. 
% \winston{FRAMING cut this, belongs in sec 3}
% Each stage has various methods, and each combination of methods from 2 stages leads to an approach to output circuits for an input Hamiltonian.
% These 2 stages are optimized independently, which can lead to potential suboptimalities. 
% Existing workflows decompose the process into multiple stages, and improvements in one stage do not necessarily lead to better final results.
\begin{comment}
For example, the fermion-to-qubit mapping stage often focuses on reducing Pauli weight, while the smaller Pauli weight does not necessarily lead to smaller gate count or depth in later stages. \{This is redundant\}.
\end{comment}
% This motivates an end-to-end fermion-to-circuit view of the compilation process. 
% Concretely, we fix a fermion-to-qubit mapping and design tailored synthesis techniques to output an efficient circuit by exploiting Hamiltonian structure and regularity in the fermion-to-qubit mapping. 

% \fixit{A more fundamental question to ask ourselves: How do we view the entire stack for compiling from a fermion Hamiltonian to physical circuit? There are multiple abstraction layers. Which layer is most important?  Or in general, the consideration of multiple layers is more important than individually (aggressively  optimizing any single layer)? This may naturally lead to the idea of a vertical optimization from the perspective of exploiting Hamiltonian structure, regularity in fermion-to-qubit mapping,s logical circuit optimization, and hardware mapping, which is the tenet of this paper. }


% Based on these insights, we adopt the JW mapping as the starting point and develop specific algorithms to optimize the circuit synthesis result.

% \textbf{Observation 1: Scalability is an issue.}
% Our empirical study shows that, regardless of the combination choice of fermion-to-qubit mapping and circuit synthesis method, both gate count and circuit depth scale at least as O($n^5$) (shown in Figure~\ref{fig:Scalability}). 
% This rapid growth poses a scalability challenge. 
% In quantum systems, noise accumulates proportionally with circuit depth and gate count; as the problem size increases (e.g., complex molecular systems), the resulting circuits become increasingly noise-prone, leading to a degradation in computational accuracy.

% The approach proposed in this paper can achieve O($n^4$) outcome, orders of magnitude better than the state-of-the-art.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{EvaluationFigures/complete_vs_excitations.png}
    \vspace{-0.1in}
    \caption{Gate count and depth normalized to number of 2nd excitation terms for all-to-all Hamiltonians on Linear architecture. State-of-the-art have superlinear scaling compared to number of second excitation terms. \sysname{} is more scalable and is the best for $\ge 11$ qubits.
    }
    \label{fig:ScalabilityA2A}
\end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{EvaluationFigures/complete_depth_vs_excitations.png}
%     \vspace{-0.1in}
%     \caption{Circuit depth normalized to number of 2nd excitation terms for all-to-all Hamiltonians on Linear architecture. State-of-the-art have superlinear scaling compared to number of second excitation terms. \sysname{} is the best for $\ge11$ qubits. 
%     }
%     \label{fig:ScalabilityDepth}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.49\textwidth]{EvaluationFigures/complete_log_cx.png}
%     \vspace{-0.1in}
%     \caption{Log-log plot of CNOTs against qubit count for complete Hamiltonian case, targetting Boston.}
%     \label{fig:complete_log_cx}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.49\textwidth]{EvaluationFigures/complete_cx.png}
%     \vspace{-0.1in}
%     \caption{State-of-the-art approaches faces scalability issues, using at least $\Omega(n^5)$ hardware circuits.\xiangyu{Maybe divide by $n^3$ is not quite useful. BTW, I am considering that Fig 2 can show depth over $n^4$, depth over $n^5$ instead of \# CNOTs and Fig 3 can show \# CNOTs}}
%     \label{fig:Scalability}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.49\textwidth]{EvaluationFigures/complete_cx_vs_excitations.png}
%     \vspace{-0.1in}
%     \caption{Scaling comparing 2nd excitation terms of complete Hamiltonian vs CNOT count for state-of-the-art compilers.}
%     \label{fig:Scalability}
% \end{figure}

\noindent\textbf{Observation 1: Smaller Pauli weight in fermion-to-qubit mapping does not necessarily lead to smaller depth and gate count in qubit-to-circuit synthesis and hardware mapping results.} 
% \winston{TODO add figure for Linear JW/BK Tet/PH total gate count. show JW beats BK (wow) QUALIFY THIS IS TOY CASE Fig~\ref{fig:misc_pauli_weight}}
% \xiangyu{Check with Winston, if we decide to use Figure~\ref{fig:complete_log_cx}, where do you think is a good place to mention?}
Existing approaches typically optimize in a step-by-step manner, where the first stage focuses on improving intermediate metrics such as Pauli weight, under the intuition that lower Pauli weight implies lower hardware cost. 
However, this intuition does not always hold. 
% for both gate count and circuit depth by varying the problem size in . 
Figure~\ref{fig:misc_pauli_weight} shows that in several benchmarks, BK mapping with smaller Pauli weights produces results with larger gate count than (or similar to) JW mapping under the same circuit synthesis method (e.g., Paulihedral). 
Figure~\ref{fig:ScalabilityA2A} contains the result that as the number of qubits $N$ increases, 
the number of second excitation terms in all-to-all Hamiltonians scales as $O(N^4)$. 
The gate count and circuit depth produced by existing approaches grow significantly faster than $O(N^4)$. 

\begin{comment}
In contrast, \textit{our end-to-end method achieves an order-of-magnitude improvement, exhibiting near-constant scaling when normalized by $N^4$}. [Eddy: this has nothing to do with the observation, I suggest moving it to the very end of the motivation section.]
\end{comment}
% \winston{I feel we should say: showing theoretically improvement is possible, and only talk about our approach after we introduce it.}

\begin{figure}[t]
    \centering
\includegraphics[width=0.45\textwidth]{EvaluationFigures/misc_jw_vs_bk.png}
\vspace{-0.1in}
    \caption{UCCSD benchmarks run on Linear architecture. BK generates pauli strings with smaller pauli weight than JW but the final compilation results on several benchmarks have larger gate count in the linear architecture.
    % in linear architecture.
    }
    \label{fig:misc_pauli_weight}
\end{figure}

\begin{figure}[t]
    \centering
\includegraphics[width=0.49\textwidth]{Figures/BK.pdf}
    \vspace{-0.4in}
    \caption{Comparison of the double excitation form of Pauli operators generated by the Jordan–Wigner (JW) and Bravyi–Kitaev (BK) mappings. (a) JW mapping uses a linear (degenerate) ternary tree; (b) BK mapping adopts a ternary-tree-based structure.
    For a 4-qubit example, we enumerate the resulting Pauli operators under each mapping.
    JW produces Pauli strings with a more regular pattern than BK.
    }
    \label{fig:BK}
\end{figure}

% This is largely because Tetris' heuristics are more compatible with JW mapping's outcome, meaning that sometimes optimizing intermediate objectives can mismatch with downstream synthesis heuristics. 
% \xiangyu{TODO: mention }

\noindent\textbf{Observation 2: The Jordan--Wigner (JW) mapping generates Pauli operators with more regular structures.} 
% \xiangyu{Try to leverage my result to see the regularity of JW and non regularity of BK}
% \fixit{Given Winston's new data, JW does not present the most benefit anymore. How about we modify this to that JW has more regularity than BK -- using the example that Xiangyu made earlier, or we brainstorm together?} 
% We evaluate a diverse set of fermion-to-qubit mappings and compare their resulting circuit synthesis performance. 
% Our empirical evaluation shows that the Jordan-Wigner mapping achieves lower gate count and circuit depth compared to alternatives. 
% To generate the Pauli operators, 
Different mappings choose different strategies to encode fermionic information into Pauli operators.
In the JW mapping, each fermionic operator is translated into a Pauli string with a linear prefix structure, while the BK mapping relies on a tree-based parity encoding (e.g., Fenwick trees).
As a result, JW produces Pauli operators with regular patterns due to its linear structure, whereas the operator structure generated in BK  depends on the specific tree construction and node indexing and is less uniform. 
Figure~\ref{fig:BK} illustrates this using a 4-qubit example: operators produced by JW have 
% produces 8 operators \winston{CLARITY everyone does 8. can drop} with the same length with 
a regular, predictable pattern, but those output by BK are more irregular and scattered.

% We further analyze the Pauli strings generated by different mappings. 
% We observe that while most mappings exhibit structured operator patterns, patterns produced by the Jordan-Wigner mapping are more amenable to our circuit synthesis procedure. 

% Bring more gate cancelation opportunities to quantum toplogies where contain a straight line passing most of (if not all) qubits.

% \winston{Move Linear hardware path observation here}
\noindent\textbf{Observation 3: The widely existing linear path connectivity across quantum hardware can be utilized to optimize the circuit compilation.} 
Although different quantum devices exhibit various hardware topologies, a linear path that passes through most (if not all) of the device's qubits is a common pattern (as shown in Appendix~\ref{appendix:linear-pattern}). Moreover, a linear path is the most restricted form of hardware connectivity. Hence, if one can compile a Hamiltonian into a linear architecture, the compilation strategy will work for nearly all recent hardware platforms. 
Existing circuit compilers take into account an arbitrary target hardware topology and rely on heuristics to produce the compilation result. 
Their solutions are more general. However, it may miss opportunities for optimizations via hardware topology specialization. Based on our observation of the expanded Pauli-operator double excitation form in equation~\ref{eq:jw-pauli} in Section \ref{approach}, the Pauli-exponential output by JW typically have a contiguous Z-prefix structure, which may directly be embedded onto a linear qubit layout. This inspires our further exploration of choosing JW as the main fermion-to-qubit encoding approach together with the linear connectivity as the foundation of this research study. 

\textit{Our end-to-end method on this foundation achieves an order-of-magnitude improvement, exhibiting near-constant scaling when normalized by $N^4$} which none of the state-of-the-art approaches can achieve, as shown in Appendix~\ref{appendix:scalability}.

% \winston{FRAMING path is observation 4. no one has talked about this before, we should distinguish}
% Beyond these observations, we find that across various quantum device topologies, it is easy to find a straight line (called Hamiltonian Path~\cite{hamiltonianPath}) where most (if not all) of the qubits sit on that path (shown in Figure~\ref{fig:linearCommon}).  
% \winston{CLARITY explicitly say why we even bother with each of these choices.}ji

% \winston{FRAMING on different cases, no one compiler is the best. if we optimize for specific problem (UCCSD, material), we may be able to do better. for me: Configuration space problem. Figure~\ref{fig:misc_comparison}}




\noindent\textbf{Observation 4: Lack of vertical stack integration in existing Hamiltonian compilation approches.} 
% \fixit{Is this surprising?} Linear connectivity is a commonly used abstraction for quantum devices. \fixit{How about we say a vertical stack integration is better than individually optimizing each layer in the software stack, rather than most architectures have an embedding of a line architecture?}}
Prior approaches typically adopt a multi-stage pipeline where each stage is operated in an isolated manner from fermionic Hamiltonians to circuits (shown in Figure~\ref{fig:CircuitSynthWF}). 
Each stage of this pipeline has a specific objective to optimize (e.g., the Pauli weight in the fermion-to-qubit stage). 
This forces later stages to be able to handle a wide variety of outputs from previous stages. 
Potential suboptimalities occur to support such generality. 
% To support such generality, these synthesis algorithms are typically heuristic-based.
This multi-stage design produces several compilation paths from the initial fermion Hamiltonian to the finally generated circuits (e.g., JW+Paulihedral, JW+Tetris, BK+Tetris). 
As shown in Figure~\ref{fig:misc_comparison}, there is no single path that can dominate all others. For instance, Tetris+BK's compilation outcome is best for the C2F2 molecule but becomes the worst for the C4H4N2 molecule. 
Users are required to test all these combinations if they want to get the best compilation result.  
To remedy this problem, we believe a vertical integration of all stages can bring global optimization opportunities and simplify users' tasks of choosing the best combination along the multi-stage pipeline. 


\begin{figure}[t]
    \centering
\includegraphics[width=0.45\textwidth]{EvaluationFigures/misc_comparison.png}
    \caption{Various benchmarks run on Linear architecture. Total gate count normalized to average of compilation pipelines. NO BEST combination solution in different stages in the compilation pipeline.
    }
    \label{fig:misc_comparison}
\end{figure}

\textbf{Takeaway Message:} 
Due to the nature of the multiple-stage pipeline of compiling Hamiltonian simulation applications, there are many possible pathways. Due to the regularity in JW and our empirical experiment results, we consider the particular pathway of starting with the JW mapper as the most promising. Our exploration in fact demonstrates that it brings us significantly more opportunities than the other potential pathways in this two-stage compilation process.

This begs the question: As researchers are working independently on different abstraction layers of Hamiltonian simulation, how does each abstraction layer's result affect the next abstraction layer? Our main takeaway message is that fermion-to-qubit mapping, may not need extensive exploration. For as what we can see, through our Accordion approach using JW, we can achieve circuit complexity of $O(N^4)$, however, for the optimal fermion-to-qubit mapping approach BK, it requires $O(\log(N))$ for average weight of Pauli-operators, and in total, it requires $O(N^4)$ terms, bringing it to at least $O(N^4*\log(N))$ overall circuit complexity without considering hardware routing overhead. However, in practice, BK's performance is actually on par with $O(N^5)$ in Figure \ref{fig:ScalabilityA2A} through empirical experiment results. This demonstrates that further research on reducing the Pauli-weight in fermion-to-qubit mappings may not be necessary, as it is unlikely to beat the $O(N^4)$ complexity of Accordion's result for at least the full rank electronic structure Hamiltonians.  
 

% In contrast, an end-to-end (vertical) integration that the compiler to specialize for the resulting Pauli operator patterns. 
% When the mapping exhibits regularity (e.g., in JW), it becomes possible to design tailored circuit synthesis techniques that systematically exploit such structures, 
% leading to improved optimization opportunities in metrics such as gate count and circuit depth.


% \noindent\textbf{Observation 4: Missing end-to-end optimization opportunities.} 
% A fundamental limitation of state-of-the-art approaches is the strict decomposition of the fermion-to-circuit compilation process into multiple stages. 
% In particular, circuit synthesis methods in the second stage are designed to be generic, so that they can accommodate the outputs of various fermion-to-qubit mappings. 
% This generality comes at the cost of missing opportunities for customized optimization. If the mapping is fixed, it becomes possible to exploit its structural properties and co-design the circuit synthesis procedure accordingly, enabling end-to-end optimization across the entire pipeline. 




==> related.tex <==
\section{Related work}
\label{sec:related}

\Para{Multi-stage process to generate circuits for Fermionic Hamiltonians.} 
Previous approaches divide the circuit generation into multiple stages. 
First of all, works such as JW~\cite{JW}, BK~\cite{BK}, HATT~\cite{hatt}, and Fermihedral~\cite{Fermihedral} produce Pauli strings with various Pauli weights. 
Bonsai algorithm~\cite{bonsai} is developed to output a tailored fermion-to-qubit mapping from ternary trees. 
Then, works such as Tetris~\cite{Tetris}, Paulihedral~\cite{Paulihedral} take as input the Pauli strings and output the quantum circuit for execution in target hardware devices. 
Contrary to this design, \sysname{} unifies the whole process by fixing the choice of JW mapping and designing a tailored circuit synthesis algorithm to improve the gate count and circuit depth. 


\Para{Optimizations in Quantum Compilers.}
State-of-the-art quantum compilers (e.g., Qiskit~\cite{qiskit}, Cirq~\cite{cirq}, Braket~\cite{braket}) incorporate passes such as gate cancellation~\cite{nam2018automated} and qubit routing~\cite{pozzi2022using} to optimize quantum circuits. 
They can be applied to circuits generated after the fermion-to-circuit process completes. 
\sysname{}'s framework can be complementary to these optimizations of quantum compilers.
